Concept-free Causal Disentanglement with Variational Graph Auto-Encoder

In disentangled representation learning, the goal is to achieve a compact representation that consists of all interpretable generative factors in the observational data. Learning disentangled representations for graphs becomes increasingly important as graph data rapidly grows. Existing approaches often rely on Variational Auto-Encoder (VAE) or its causal structure learning-based refinement, which suffer from sub-optimality in VAEs due to the independence factor assumption and unavailability of concept labels, respectively. In this paper, we propose an unsupervised solution, dubbed concept-free causal disentanglement, built on a theoretically provable tight upper bound approximating the optimal factor. This results in an SCM-like causal structure modeling that directly learns concept structures from data. Based on this idea, we propose Concept-free Causal VGAE (CCVGAE) by incorporating a novel causal disentanglement layer into Variational Graph Auto-Encoder. Furthermore, we prove concept consistency under our concept-free causal disentanglement framework, hence employing it to enhance the meta-learning framework, called concept-free causal Meta-Graph (CC-Meta-Graph). We conduct extensive experiments to demonstrate the superiority of the proposed models: CCVGAE and CC-Meta-Graph, reaching up to $29\%$ and $11\%$ absolute improvements over baselines in terms of AUC, respectively.

==> backup/method_01_19.tex <==


\section{Causal Disentanglement Analysis in VAEs}

\textcolor{blue}{To improve readability, maybe it's better not to introduce theory first. I have an idea: how about introduce our method first, and introduce these theory, to say like "We propose a method to solve sub-optimality in VAEs. Secondly we prove why we can solve it...}

%因为VGAE属于VAE是一个特例，二者逻辑一致，所以我们从一般情况着手/


As discussed above, existing solutions for VAE tend to offer suboptimal latent representations.
We now offer a theoretical analysis of causal disentanglement in VAE regarding optimal solutions. 
Specifically, we aim to answer the following questions: 1) is there an optimal latent representation that makes the approximated observation distribution the same as the true observation distribution while attaining the true generate factors $Z^*$,
%\textcolor{blue}{LIN: it is not enough here, disentanglement learning aims not only to make approximated distribution equal to the true distribution(it is easy to realize), but also to find out the true generate factors(here is $Z^*$, in other words, make $G=Z^*$},
and 2) how to find such a representation if it exists?




We start by showing that in a casual setting and under some mild assumptions, the causal disentanglement suggested by our theory must induce an optimal solution that makes the equation of  $p_{\theta}(X)=p^{*}(X)$ always true, aiming for the first question.
%As mentioned above, the suboptimality issue in VAEs is due to the divergence between the optimal distribution and inferred data distribution.
Before detailing the proposed main theorem, we first introduce the following proposition:
\begin{prop}
\label{prop_1}
Based on the DCP, the inferred data's distribution is as follows:
\begin{equation}
\label{G2X}
p_{\theta_{\zeta_x}}(X)=\int_{G}p_{\theta_{\zeta_x}}(X|G)p(G)dG,
\end{equation}
where we summarize the process~(\ref{C}) and~(\ref{G}) in the DCP definition as $ G=Q({\zeta}^{+})$, with $\zeta_G=\{\zeta_1,\zeta_2,...,\zeta_m\}$ and $ \zeta^{+}={\zeta_C}\cup {\zeta_G}$.
\end{prop}




\eat{
Before detailing the proposed main theorem, we first introduce two necessary lemmas.
\begin{lemm}
\label{L1}
$\forall$ K dimension continuous variable $X=(X_1,...,X_K)$, if the support set of its joint probability density is a convex set in $R^K$, then $\exists$ K dimensional independent uniform variables $U=(U_1,...,U_K)$ and a set of function $F=\{f_1,f_2,...,f_K\}$ result in $X=F(U)$ that $X_k=f_k(U_1,...,U_k)$.
% \todo{following is unclear}
% for each one we have $X_k=f_k(U_1,...,U_k)$ with $k\in[1,2,...,K]$. 
\end{lemm}



The proof of Lemma~\ref{L1} is provided by~\citet{HePing}. 
The above lemma indicates that it is possible to represent continuous observations with convex joint density distributions by projecting a list of independent variables onto some functions.
{We now present the following lemma showing that any given continuous variable can be associated with a uniform distribution.}


\begin{lemm}
\label{L2}
$\forall$ continuous variable $X$, set its distribution function as $f(X)=P(X \leq x)$, then $f(X) \sim U(0,1)$. 
\end{lemm}



\begin{proof}
$P(f(X) \leq a)=P(X \leq f^{-1}(a))=f(f^{-1}(u))=a$, where $a$ is a constant.
\end{proof}
}

%Based on these two lemmas, we can acquire such a theorem:
%\begin{theo}
%\label{T1}
%$\forall$ $K$ dimension continuous variable $Z=(Z_1,...,Z_K)$, $\exists$ $K$ dimentions independent normal variables $N=(N_1,...,N_K)$ and set of function $Q=\{q_1,...,q_K\}$, $Z=Q(N)$ and $Z_i=q_i(N_1,...,N_i)$, $i=1,2,...,K$. 
%\end{theo}
%\begin{proof}











\eat{
\textcolor{blue}{
To simplify the process (\ref{G}) and (\ref{C}): note that $H_{i}^{C}$ is function of $N_C$, then $G_i$ is function of $N_C,N_1,N_2,...,N_m$. Formally, we set $N_G=\{N_1,N_2,...,N_m\}$ and $ N^{+}={N_C}\cup {N_G}$.}
Without losing generality, we can simplify the process (\ref{G}) and (\ref{C}) as:
\begin{equation}
\label{Q'}
G=Q_G(C({N_C}), {N_G}) \rightarrow G=Q(N^{+}) 
\end{equation}
where $N_C$ and ${N_G}$ are independent normal variables as prior, %$Q'$ represents set of $f$ in (\ref{G}), 
and $Q_G=\{q_1,q_2,...,q_m\}$. % we can denote (\ref{Q'}) as:%\todo{why?}
%\begin{equation}
%\label{Q}
%G=Q(\mathbf N)
%\end{equation}
\textcolor{blue}{The process (\ref{X}) is to acquire $X$ by $G$ and $N_x$, where $N_x$ is noise variables. So we could assume the distribution of $X$ as: }%\todo{why we need this? }
\begin{equation}
\label{G2X}
p_{\theta_{N_x}}(X)=\int_{G}p_{\theta_{N_x}}(X|G)p(G)dG
\end{equation}

}












The proof of Proposition~\ref{prop_1} is at Appendix~\ref{}.\textcolor{blue}{It may be more like an assumption?}
In this way, we can formulate the data distribution by using the causal generative factor $G$, which is graph-structured, in contrast to using the independent variable-based representation  $Z$ in traditional VAEs.
Using this causal generative factor allows us to circumvent the sub-optimality problem caused by the independent constraint in previous latent representation learning.
However, a key challenge remains on how to prove the existence of function $Q$ in Equation~\ref{G2X} so that the obtained representation $G$ can ensure the equivalence between two data distributions, i.e.,  $p_{\theta_{\zeta_x}}(X)=p^{*}(X)$, and the optimality of $G$, i.e., $G=Z^{*}$.
To address this, we propose our first main theorem, namely:
\eat{
we can thus reformulate the distribution of $X$ as $p_{\theta_{G}}(X)=\int_{G}p_{\theta_{G}}(X|G)p(G)dG$ 
% \textcolor{blue}{LIN: I think we don't need to rewrite the distribution of $X$ again cause we have claimed it in equation \ref{G2X}, but stress the difference from VAE is important, how about cite equation \ref{G2X} instead of rewriting here?} 
in contrast to using the independent variable-based representation $Z$ in traditional VAEs.

We now theoretically investigate why causal disentanglement leads to an optimal solution while holding $p_{\theta_{G}}(X)=p^{*}(X)$.


Essentially, we need to prove the existence of function $Q$ in Equation~\ref{G2X}, guaranteeing that above two distributions are equivalent, as shown in the following theorem.
}
% \textcolor{blue}{In other words, is there exist such $Q$ in equation \ref{Q'} that garantee the  $p_{\theta_{G}}(X)=p^{*}(X)$?}
%  by proposing our main theorem




% Recall that DCP provides a path from causes $G$ to observations $X$, we thus can reformulate the corresponding distribution as $p_{\theta_{G}}(X)=\int_{G}p_{\theta_{G}}(X|G)p(G)dG$ as opposed to using independent variable-based representation $Z$ in traditional VAEs.



% We now propose our main theorem that causal disentanglement results in an optimal solution for the VAEs.
\begin{theo}
\label{P1}
 Given independent Normal distributed variables $ N=\{N_1,...,N_K\}$, there exists a causality modeling function $Q$ that represents the causal generative factor $G=\{G_1,...,G_K\}$ that $G_i=Q_i(N_i^S)$, resulting in following equivalences: 1) $p_{\theta_{\zeta_x}}(X)=p^{*}(X)$ and 2) $G = {Z^*}$,
 % \textcolor{blue}{No need of $G = {Z^*}$, we can prove that there exist $G=Q(N)$ making $G=Z^*$},
 with $ p^{*}(X)=\int_{Z^*}p^{*}(X|Z^*)p^{*}(Z^*)dZ^*$,  where $p^{*}(Z^*)\neq \prod_{i}p(Z^*_i)$.
 Here, $N_i^S$ is a subset of $N$.
% under conditions 
% of (\ref{p*}) and (\ref{G2X}).
%\textcolor{blue}{LIN: I have do some change about the dimension of N and G. I want to distinguish N in Definition 3.1 and Theorem 4.1, they are two different N. In Definition 3.1, N is given in causal graph, but in Theorem 4.1, N is arbitrary independent normal distribution, so they may have different dimension (m and K). }
\end{theo}

We defer the proof of Theorem~\ref{P1} to the Appendix~\ref{App1}.
Theorem~\ref{P1} provides a positive answer to question (1), i.e., in a casual setting, there exists an optimal solution for VAEs.




\eat{
\begin{proof}
\todo{this  need to be moved to appendix}

Generally speaking, proving Theorem~\ref{P1} equala to finding functions $q_i$, $i=1,2,...,K$ that make $G_i=q_i(N_1,...,N_K)=C_i$ true.
We now present the proof in four steps as follows.

Step 1: Because of Lemma\ref{L1}, we get that there exists independent uniform variables $(U_1,...,U_K)$ and function $F$ make $C=F(U)$, in which:
\begin{equation}
    U=(U_1,...,U_K)
\end{equation}
\begin{equation}
\label{fi}
    C_i=f_i(U_1,...,U_i)
\end{equation}

Set $U_i \sim U(a_i,b_i)$, $i=1,2,...,K$.

Step 2: Set there are arbitrary K independent normal variables $N_1,...,N_K$, $N_i \sim N(\mu_i,\sigma^2_i$). Set distribution function of $N_i$ is $g_i$, which means $g_i(x)=P(N_i \leq x)$. Denote:
\begin{equation}
\label{U'i}
    g_i(N_i)=U'_i, i=1,2,...,K
\end{equation}


Step 3: Because of Lemma\ref{L2}, $U'_1,...,U'_K$ are independent and they all are variables of uniform distribution $U(0,1)$.

Then $U_i$ in Step 1 can be represents by $U'_i$ as:
\begin{equation}
    U_i=(b_i-a_i)U'_i+a_i, i=1,2,...,K
\end{equation}
Because $g_i(N_i)=U'_i$ in (\ref{U'i}), which means $U'_i$ is function of $N_i$, so we can denote:
\begin{equation}
\label{hi}
    (b_i-a_i)U'_i+a_i=h_i(N_i)
\end{equation}


Step 4: Then we can find $C_i=q_i(N_1,...,N_K)$ as:
\begin{equation}
\label{qi}
    C_i=f_i(h_1(N_1),h_2(N_2),...,h_i(N_i))\\
    =q_i(N_1,...,N_K)\\
\end{equation}
In which set of $f_i$ is from equation \ref{fi} and $h_i$ is from equation \ref{hi}. Therefore, we can induce Theorem~\ref{P1} is right because $\forall$ $C$ (in equation (\ref{p*})), $\exists$ a function $Q$ makes $G=Q(\mathbf N)=\{q_i(N_1,...,N_K)\}_{i=1,2,...,K}$ (from equation (\ref{qi})) is equal to $C$ .

\end{proof}
}








%this can be extended to a more general conclusion, as shown in Appendix~\ref{}.


\eat{
\todo{why we need this? never being used later on}
\begin{remark}
\label{remark1}
$\forall$ $K$ dimension continuous variable $Z=(Z_1,...,Z_K)$, $\exists$ $K$ dimensions independent normal variables $N=(N_1,...,N_K)$ and set of function $Q=\{q_1,...,q_K\}$, $Z=Q(N)$ and $Z_i=q_i(N_1,...,N_i)$, $i=1,2,...,K$.
\end{remark}
The proof of Remark \ref{remark1} is in appendix.
}
%%%%%%%%
%%%%%%%%
%%%%%%%%
%With Theorem~\ref{T1}, we can induce Theorem~\ref{P1} because $\forall$ $C$ in (\ref{p*}), $\exists$ a function $Q$ (from Theorem~\ref{T1}) makes $G=Q(N)$ (in equation(\ref{G2X})) is equal to $C$.


%\end{proof}




\subsection{Causality Modeling Function Properties}\label{how to get Q}
%\todo{ set }\\

In the last section, we proved the existence of a causality modeling function to gain an optimal solution for VAEs.
% We now offer analysis on how exactly do we go about designing function $Q$ in Theorem~\ref{P1}.
% We now offer an analysis of how exactly we go about the construction of the $Q$-function in Theorem~\ref{P1} under the context of causality.




% In the following, we outline principles for designing this function, as shown in Theorem~\ref{conditions}.


% According to Theorem~\ref{P1}, we know the optimal representation $G$ depends on independent normal distributed variables and a causality modeling function.
% % With the goal of finding optimal $G$, we will need to find a function $Q$ and variables $N$ to ensure the optimality of $Q(N)$. 
% At a high level, finding optimal $G$ is to obtain function $Q$ and variables $N$ to ensure the optimality of $Q(N)$ as $G=Q(N)$. 
% % According to Theorem~\ref{P1}



% is obtained by projecting independent variables into

Firstly, we show that all independent normal distributed variables are interchangeable under linear transformations, as shown in the following theorem.

\begin{theo}
\label{conditions}
% Assuming $B  = A * {diag(N')}\in \mathbb{R}^{K \times K}$, along with the following conditions: \\
Given the following condition: 
% Condition 1:  $A \in \mathbb{R}^{K \times K}$  can be obtained by finite row-wise permutation of a lower triangular matrix;\\
$ N'$ consists of $K$ independent normal variables as $ N'=(N'_1,N'_2,...,N'_K)^T$, and set $a_i$ and $b_i$ as non-zero real numbers, 
there must exist $N_k \in N$ ( N from Theorem~\ref{P1}), such that the following equation holds: $N'_i=a_i\times N_k+b_i, i=1,2,...,K$.\\
% \textcolor{blue}{(2) Denote $Q=\{Q_1,Q_2,...,Q_K\}$(in Theorem \ref{P1}) and $Q_i^{-1}(G_i)=N^{S}_{i} \subseteq  \{N_1,N_2,...,N_K\}$, then for each $Q_i$ there must exist $Q'_m \in Q'$  and a constant diagonal matrix $V_i$ and constant vector $M_i$ such that: $Q_i^{-1}(G_i)=V_iQ'_m^{-1}(G_i)+M_i=N^{S}_{i}$ if $Q_i$  and $Q'_m$ are reversible. 
% } 
\end{theo}

% This lemma implies that data with same property, i.e., independent normal distributed, are from the same space.
Based on this theorem, we provide a new def

\begin{defi}
%( optimal solution expression?)
For simplicity, we rewrite each causal generative  factor  in Theorem~\ref{P1} as $G_i=Q'_i(B_i)$,($i=1,2,...,K$), $B_i$ is i-th row of $B$
with 
1) $B  = A * {diag(N')}$ and
2) $A \in \mathbb{R}^{K \times K}$  comes from finite row-wise permutation of a lower triangular matrix.
    $Q'_i:{N'}^S_i \longrightarrow G_i$, ${N'}^S_i \subseteq N'$.
\end{defi}




% G是最优解，所以是唯一性。
% 证明的逻辑： 假设存在不同的函数Q'，达到最优的G，最终证明，Q&Q'的映射关系一致
% 所以我们可以声称要达到最优的G，其函数Q也必然是唯一的，因为他们之间必然映射关系一致。
% 最终结论：

% 最优的 G确定 的，这个等价于说最优的 Q(N)是确定，
% 所以，改变了Q，也就是得到了Q'，我们通过定理证明了：
% 只要是满足我们的C2条件的 Q(N)(分别是Q和N，一起才行），就一定能找到和理论上最优的Q(N)之间的线性转化关系，
% 
% 两个condition能保证 原象 空间一致，我们的假设前提是我们都以 最优解为 投影象。在此基础上，
% 我们两个function的等价性，在某种条件下，我们能

% 空间等价（同一个空间）%

%  lemma2 显示了，不同Q本质上是在同一个投影空间，因为他们的投影是 affine transformation，

\begin{lemm}
\label{lemma_space}
For each optimal projection $Q_i$ in Theorem~\ref{P1},
there must exist and only exist one $Q'_i$ % \in {Q'_1,Q'_2,...,Q'_K}$ 
under the context of Definition 4.1 share the same projection space to obtain the optimal representation $G_i$, i.e., $space({N'}^S_i) =  space(N_i^S)$.
% there must exist $Q'_j \in Q'$  and a constant diagonal matrix $V_i$ and constant vector $M_i$,
% such that: $Q_i^{-1}(G_i)=V_iQ'_j^{-1}(G_i)+M_i=N^{S}_{i}$ if $Q_i$  and $Q'_m$ are reversible. 
\todo{Q-k or Q-i? }
\end{lemm}



Lemma~\ref{lemma_space} suggests that 
as long as the projection space is the same, 
we can always get:
All vectors in $space(N_i^S)$ can be acquired by one of rows of $B$
%in $A * {diag(N')}$, 
%means that each row of $Q(A * {diag(N')})$ is one and only one of $Q_1(N^S_1), Q_2(N^S_2),...,Q_K(N^S_K)$ 
$\longrightarrow$ we can use $Q'(A * {diag(N')})$ to find $G_i$

\begin{lemm}
\label{lemma_linear}
Assume $Z^*_1,Z^*_2,...,Z^*_K$ is a linear uniform distribution as Equation~\ref{linear uniform}. When $N_i$ in Theorem~\ref{P1} is in the interval $N_i \in \left [\mu_i-\delta,\mu_i+\delta \right]$,$i=1,2,...,K$, $\delta $ is a non-negative real number, $\mu_i$ is mean of $N_i$, for each $Q_i(N^S_i)$, there exist a linear function $Q^L_i(N^S_i)$ make the absolute error has such bond:$|Q_i(N_i^S)-Q^{''}_i(N^S_i)|\le O_i( \delta)$, \\where:
\begin{equation}
\label{linear uniform}
    P(Z^*_k|Z^*_1,...,Z^*_{k-1}) \sim U(\eta_k+r_{k0},\eta_k+r_{k1}),k=1,2,...,K 
    P(Z^*_1,Z^*_2,...,Z^*k) is a uniform distribution, Z^*_k \in (c_k-\sum_{t=0}^{k-1} r_kt z^*_t, c_k+\sum_{t=0}^{k-1} r_kt z^*_t), k=0,1,...,K
\end{equation}
$\eta_k= \sum_{t=1}^{k-1} c_{kt}Z^*_t$, and $c_{k1},c_{k2},...,c_{k,k-1},r_{k0},r_{k1}$ is real number, $O(\delta)=c_{i0}+\delta\Lambda_i$,  \todo{c? xiabiao}$\Lambda_i=\frac{1}{\sqrt{2\pi}}\sum_{t=1}^{i}  c_{it}(1-e^{-\frac{\delta ^2}{2\sigma^2_t} })$, $c_{k0}=-\frac{r_{k0}}{r_{k1}-r_{k0}}$, $\sigma^2_t$ is the variance of $N_t$. 
\end{lemm}

Lemma~\ref{lemma_linear} suggests that 
$Q$ can be approximated by a linear function in an interval with the error similar to the interval length. \todo{douhao or ju hao? next sentence}(About $\delta$: in fact, it is a very small probability (less than 5\%) to make normal variables $N(\mu,\sigma)$ beyond $\left[\mu-2\sigma,\mu+2\sigma\right]$, so the error can be bonded by the same level of the max variance of $N_i,i=1,2,...,K$ with over $95\%$ probability.)
So $Q'$ can be implemented as a linear function, means:\\
$Q'(A * {diag(N')}) \rightarrow C*A'*{N'}$ is legal because:\\
$Q_i(N_1,N_2,N_3) \rightarrow a_1*N_1+a_2*N_2+a_3*N_3 \rightarrow (a_1,a_2,a_3)*(N_1,N_2,N_3)^T : (a_1,a_2,a_3)\rightarrow {A'}_i$ \\

In Lemma~\ref{lemma_linear} , we assume that $Z^*_1,Z^*_2,...,Z^*_K$ is a linear uniform distribution and we can prove in such assumption, linear function has good property. However, not every linear function is a good solution of $Q$. But we can provide an approaching idea. Because $Q_i(N^S_i)=G_i$ is designed to approach $Z^*_i$, so it is better to make $G_i$ has similar distribution to $Z^*_i$. In the assumption of $Z^*_i,i=1,2,...,K$, we can get that the conditional distribution $Z^*_k$ always determined by $Z^*_1,Z^*_2,...,Z^*_{k-1}$, $k=1,2,...,K$. So the relationships among $Z^*_1,Z^*_2,...,Z^*_K$ can be described by a directed graph where $Z^*_k$ has $k-1$ father nodes $Z^*_1,Z^*_2,...,Z^*_{k-1}$, which means that the adjacency matrix of $Z^*_1,...,Z^*_K$ is a lower triangular matrix. Therefore, we can design a similar graph for $G_1,G_2,...,G_K$ with a lower triangular adjacency matrix. (In experience, we do not have to make the index of $G_1,...,G_K$ one-to-one correspondence with $Z^*_1,...,Z^*_K$, so the adjacency matrix of $G_1,...,G_K$ only need to be a matrix which can be acquired by a lower triangular matrix with finite row exchange.) %But in practice, it is too difficult to design a constrain for adjacency matrix directly by such requirement. Fortunately, this requirement can be met by designing this graph as DAG, and constrain for DAG can be designed more conveniently. So we can make $G_1,...,G_K$ become factors in DAG)

$(I-\Phi)^{-1}\varepsilon^T=C*A*{diag(N')}$\\
% \begin{def}
%     (causal *****):
%  given ,, with,...
%  , 
%  we can get the optimal solution in Th4.1.
% as :
  
% \end{def}







\eat{
\begin{theo}
\label{conditions}
 
%Condition 1: G is not independent\\
%condition 2: Q is not injective\\
Consider a function set
$Q'=\{Q'_1,...Q'_K\}$ that computes  causal generative factors with a row-wise formulation as $G_i=Q'_i(B_i)$.
% \textcolor{blue}{here $B_i$ is the i-th row of matrix $B$, $G_i$ is i-th of $G$ in Theorem \ref{P1}}. 
Assuming $B  = A * {diag(N')}\in \mathbb{R}^{K \times K}$, along with the following conditions: \\
Condition 1:  $A \in \mathbb{R}^{K \times K}$  can be obtained by finite row exchanges of a lower triangular matrix;\\
Condition 2: $ N'$ consists of $K$ independent normal variables as $ N'=(N'_1,N'_2,...,N'_K)^T$;\\
we \\
(1) there must exist two real numbers denoted as $a_i$ and $b_i$, and exist $N_k \in N$ as in Theorem \ref{P1}, such that the following equation holds: $N'_i=a_i\times N_k+b_i, i=1,2,...,K$.\\
\textcolor{blue}{(2) Denote $Q=\{Q_1,Q_2,...,Q_K\}$(in Theorem \ref{P1}) and $Q_i^{-1}(G_i)=N^{S}_{i} \subseteq  \{N_1,N_2,...,N_K\}$, then for each $Q_i$ there must exist $Q'_m \in Q'$  and a constant diagonal matrix $V_i$ and constant vector $M_i$ such that: $Q_i^{-1}(G_i)=V_iQ'_m^{-1}(G_i)+M_i=N^{S}_{i}$ if $Q_i$  and $Q'_m$ are reversible. 
} \todo{rewrite}
\end{theo}
}



The proof is given in the Appendix~\ref{App2}.


% Theorem \ref{conditions} tells us if $Q$ satisfies two conditions, we can ensure the solution of $\mathbf N$ is at least the linear transformer of true $\mathbf N$ when equaling $G=Q(\mathbf N)$.  
\textcolor{blue}{Theorem \ref{conditions} implies any functions $Q'$ with the mentioned two conditions is guaranteed to meet the same mapping relationships with the true function $Q$, which makes $G'$ acquired by such $Q$ has the same statistical properties with the true $G$. }





\todo{connect to graph}
Note that  








\section{ Concept-free VGAE}
%\todo{This is a draft, some assumption about causal layer would be check in the future}
\label{sec5}



Building on the necessary conditions of the causality modeling function in Theorem~\ref{conditions}, we now introduce a causality-driven VGAE framework that encourages optimality in latent representation.
Our framework employs an encoder-decoder paradigm, with an encoder consisting of two components: a compression layer is supposed to obtain low-dimensional independent variables, followed by a causal layer for disentangled representation.
\todo{An overview of the proposed framework is provided in Figure~\ref{}. }




\eat{
We are given an undirected, unweighted graph $\mathcal {G = (V, E)}$ with $ n = |\mathcal V|$ nodes with features. Denote the graph adjacency matrix as a $n \times n$ matrix $A$ and the node features as a $n \times d$ matrix $X$. Denote the degree matrix of $A$ as $D$.

Now we consider to propose a method in an unweighted graph $\mathcal {G = (V, E)}$ with $ n = |\mathcal V|$ nodes with adjacency matrix $A_{n \times n}$ and the node features matrix $X_{n \times d}$.

Our method has 3 processes aiming to acquire $\mathbf N$, $G$ and $p_{\theta_{N_X}}(X)$ in Theorem \ref{P1} respectively, including encoder, causal layer and decoder.
}

{\bf Encoder.}
According to Theorem~\ref{P1}, the entire disentanglement procedure requires independent Normal distributed variables $N$ as the input for causality modelling function $Q$. We thus start by introducing the acquisition of $N$.


Within the context of Variational Auto-Encoders, including VGAEs, the latent space is spanned by independent variables with Gaussian distribution.
Inspired by this, we can obtain the desired variable set $N$ via the latent space learning process, also called as \textit{compression layer}.
Specifically, the encoder of VGAE takes the graph adjacency matrix $A$ and the node attribute matrix $X$ as inputs and produces the target latent space with the inference process as $q(\bm{\varepsilon}|(A,X))$, where  $\bm{\varepsilon}$ denotes latent variables. 
We propose to employ $\bm{\varepsilon}$ as our expected variable $N$, i.e. $N= \bm{\varepsilon}$., which matches the second condition in Theorem~\ref{conditions}. 




\eat{
we can acquire the distribution $q(\bm{\varepsilon}|(A,X))$ of latent variables $\bm{\varepsilon}$ (as equation (\ref{encoder})).% of which mean and covariance matrix are $\mu_{n \times K}=\{\mu_i\}_{i=1,2,...,n}$ and $\sigma_{n \times K\times K}=\{{diag(\sigma_i)_{K \times K}}\}_{i=1,2,...,n}$, $\sigma_i$ is $K$ dimensions vector.% Denote $\{\sigma_i\}_{i=1,2,...n}=\sigma'$, $\sigma'$ is a $n\times K$ matrix. %We can denote $\mu=\{\mu_i\}_{i=1,2,...,n}$, in which $\mu_i$ is $K$ dimensions vector., the covariance matrix is diagonal matrix, then $\sigma$ can be represented by $\sigma=\{{diag(\sigma_i)_{K \times K}}\}_{i=1,2,...,n}$, in which $\sigma_i$ is $K$ dimensions vector. We denote $\{\sigma_i\}_{i=1,2,...n}=\sigma'$, then $\sigma'$ is a $n\times K$ matrix, which could absolutely determine $\sigma$. 
}

\eat{
  Moreover, $\varepsilon_i$ can satisfy the Condition 2 in Theorem \ref{conditions}, because the covariance matrix of each $\varepsilon_i$ is diagonal matrix, which makes them independent $K$ dimensions variables. 
  Then $\mathbf N$(in Theorem 4.1) could be acquired by $\bm{\varepsilon}$ as $\mathbf N=(N_1,N_2,...,N_K)=\bm{\varepsilon}$. \todo{??? no idea....need to remove}
  }
 
% {\bf Causal layer.}






After obtaining the required variable $N$, we develop a \textit{causal layer} to perform causal generative factor acquisition, transforming independent variables $\bm{\varepsilon}$ into a causal structured $G$.

Let $\Phi\in \mathbb{R}^{K \times K}$ be the DAG adjacency matrix for causal structure, we can present the causal generative factor $G$ using the SCM paradigm as follows,
 \begin{equation}
 \label{model_scm}
\begin{aligned}
% \label{G=C G+e}
{G}^T = \Phi^T{G}^T + \varepsilon^T \rightarrow {G}^T =(I-\Phi^T)^{-1}\varepsilon^T,
\end{aligned}
\end{equation}
where ${G}^T $ is the transpose of $G$.
\todo{...........}

Note $\Phi$ is a parameter to be learnt in the causal layer. 
Now we can prove that the $(I-\Phi^T)^{-1}$ can satisfy Condition 1 in Theorem \ref{conditions}. The proof is given in the Appendix~\ref{Proof3}
%\todo{prove in appendix}







{\bf  Decoder.}
At a high level, the goal of the decoder is to reconstruct observations from the obtained latent space. 
Given the obtained $G$, an ideal decoder is to regenerate the adjacency matrix $A$ and node attributes $X$, approximating the distribution of observations as $p_{\theta_{G}}(X)$.


\eat{
This process aims to acquire $p_{\theta_{N_X}}(X)$ in Theorem \ref{P1}, which is to regenerate the adjacency matrix and features in graph $\mathcal {G = (V, E)}$. The process to regenerate the adjacency matrix is similar to Decoder of Variational Graph Auto-Encoder as equation (\ref{decoder}). Denote $G_i$ as the $i-th$ column in $\hat{G}$, $i=1,2,...,n$.
}
%\begin{equation}
%\begin{aligned}
%p(A \mid \hat{G})=\prod\prod   p\left(A_{j} \mid \hat{G}_{i}, %\hat{G}_{j}\right)
%\end{aligned}
%\end{equation}
More specifically, we derive the edge inference and node attributes approximation as follows,
%\textcolor{blue}{LIN: these two $\sigma$ are not the same one, please make some difference between them.}
 \begin{equation}
\begin{aligned}
\begin{cases}
p\left(A_{i j}=1| {G}_{i}, {G}_{j}\right)=\sigma_1\left({G}_{i}^{T} \hat{G}_{j}\right) \\
p(X \mid {G})= \sigma_2{(G})
\end{cases}
\end{aligned}
\end{equation}
where $G_i$ is the $i$-th column of $\hat{G}$ with $i=1,2,...,n$;  $\sigma_1(\cdot)$ and $\sigma_2(\cdot)$ are  activation functions. 
Note that to avoid introducing additional parameters to the learning process and focus on studying the effect of causality, we simply use an activation function to get the value of $X$.
In particular, we employ an Exponential Linear Unit (ELU) given the mean of its output close to zero, aligned with our assumption on $X$.\textcolor{blue}{and sigmoid for $\sigma_1(\cdot)$ (same as GVAE)}


% \textcolor{blue}{ELU  is more robust and the mean is near to 0, which is more suitable for our assumption of $X$.}

%  ELU得到均值为0， ELU更合适
%X 与 G的符号的一致性

\eat{
\todo{what this is for?}
Regeneration of features is given by a nonlinear function, here we adopt an activate function:
 \begin{equation}
\begin{aligned}
p(X \mid \hat{G})= Elu(\hat{G})
\end{aligned}
\end{equation}
}


\subsection{Optimization Objective}

Till now, we present the details of the proposed framework, including an encoder and a decoder.
As with other VAEs, the optimization of this work is to encourage an equivalence between the approximated distribution $p_{\theta_{G}}(X)$ and the optimal one $p^{*}(X)$.
% Specifically, the evidence lower bound (ELBO) is used to minimize the difference between above two distributions, and to enforce  $\varepsilon$ to be independent Gaussian distribution as follows,
In particular, the evidence lower bound (ELBO) is used to minimize the divergence between the above two distributions, and to enforce that the distribution of  $\varepsilon$  is independent Gaussian, as follows,
% We adopt the ELBO band to shrink reconstruction loss between $p_{\theta_{N_X}}(X)$ and $p^{*}(X)$, and make $\varepsilon$ close to independent normal distribution:
\begin{equation}
\begin{aligned}
\footnotesize
&\mathcal{L}_G=E_{q(\hat{G}|A,X)}log(p(A|\hat{G}))+ KL(q(\bm{\varepsilon}|(A,X))|N(0,I))\\
\end{aligned}
\end{equation}

Recall that the decoder reconstructs observations from given latent representations.
Apart from minimizing distribution divergences, we also want to shorten the distance between the observation and the recovered one by measuring the mean squared error (MSE), written as:
 \begin{equation}
\begin{aligned}
\mathcal{L}_{MSE} = MSE(X,p(X|\hat{G}))
\end{aligned}
\end{equation}
 
Meanwhile, performing causal structure modeling demands a DAG constraint on $\Phi$. For the convenience of optimization, we impose a differentiable constraint function~\citep{yu2019dag} as follows, 
 \begin{equation}
\begin{aligned}
\label{DAG constrain}
\mathcal{L}_{\Phi} = tr((I-\frac{r}{K}\Phi\circ \Phi)^K)-K
\end{aligned}
\end{equation}
where $r$ is an arbitrary positive number, $tr(\cdot)$ denotes trace norm and $K$ denotes the number of concepts. 
%\todo{define m,n HERE}\textcolor{blue}{I have checked the paper of causalVAE but I can not find information of m and n, so I check the cited paper \citep{yu2019dag}, which implied m and n is the dimension of DAG, here is K exactly.}
Combining the above loss functions, we derive the overall loss function as follows,
 \begin{equation}
\begin{aligned}
\mathcal{L}=-\mathcal{L}_G+\alpha \mathcal{L}_{\Phi}+\beta \mathcal{L}_{MSE},
\end{aligned}
\end{equation}
where $\alpha$ and $\beta$ are hyper-parameters.














% \begin{thebibliography}{00}
%     \bibitem{b1} F. Träuble et al., “On Disentangled Representations Learned from Correlated Data,” p. 12.
%     \bibitem{b2} R. Suter, Ð. Miladinovic, B. Schölkopf, and S. Bauer, “Robustly Disentangled Causal Mechanisms:  Validating Deep Representations for Interventional Robustness,” p. 10.
%     \bibitem{b3} He Ping. Independence Decomposition of Multidimensional Random Variables[J]. Proceedings of the 12th Annual Academic Conference of China Field Statistics Research Association, 2005

% \end{thebibliography}


==> tex/3_method_2.tex <==


\section{Concept-free causal representation}






{\bf Problem Statement.}
Our system receives 




Often, we observe correlation in the real-world data, and formulate the corresponding data distribution as:
\begin{equation}
\label{p*}
    \begin{aligned}
      p^{*}(X)=\int_{C}p^{*}(X|C)p^{*}(C)dC,
      p^{*}(C)\neq \prod_{i}p(C_i)   
    \end{aligned}
\end{equation}
where $X\in \mathcal{R}^n$ and $C \in  \mathcal{R}^K$ are random variables, and $K \leq n$.
A classical VAE model frames the latent variable as:
\begin{equation}
    \begin{aligned}
    p_{\theta}(X)=\int_{Z}p_{\theta}(X|Z)p(Z)dZ, p(Z)= \prod_{i}p(Z_i)
    \end{aligned}
\end{equation}
where $Z \in \mathcal{R}{^K^'} $ shows random variables, and ${K^'}\leq n$.

% \textcolor{blue}{
% It has been proposed in~\cite{b1} that such process would lead to a sub-optimal solution of $p_{\theta}(X)$  equal to the optimal likelihood $p^{*}(X)$. 
% }
% \cite{b1}
%In~\cite{Frederik2020},
\citet{trauble2021disentangled} proved that this process tends to get a sub-optimal solution when equating $p_{\theta}(X)$  to the optimal likelihood $p^{*}(X)$. 

In the following, we will address this issue by using the causal disentanglement. 
%Above all, we introduce the concept of  Causal disentanglement as follows, % \cite{b2}, which could be generally described as:
% \begin{defi}
% A casual model for $X$ with generative variables $G$ and confounders $C$ is called disentanglement if and only if:
% \begin{equation}
% \label{C}
% C \leftarrow \mathbf{N_C}
% \end{equation}
% \begin{equation}
% \label{G}
% G_i \leftarrow f_i(PA_i^C,N_i),i=1,2,...,K
% \end{equation}
% \begin{equation}
% \label{X}
% X \leftarrow g(G,N_X)
% \end{equation}

% In (\ref{G}), $PA_i^C \in \{C_1, ... ,C_L\}$, $PA_i^C$ is father nodes of $G_i$ (variables in $\{C_1, ... ,C_L\}$ which influence $G_i$). $N_C, N_1, ... ,N_K, N_X$ are independent noise variables. 
% \end{defi}

Without losing generality, we can simplify the process (\ref{G}) and (\ref{C}) as:
\begin{equation}
\label{Q'}
G=Q_C(C(\mathbf{N_C}),\mathbf {N_G}) \rightarrow G=Q(\mathbf N)
\end{equation}
where $N_C$ and $\mathbf{N_G}$ are independent normal variables as prior, %$Q'$ represents set of $f$ in (\ref{G}), 
and $Q_C=\{f_1,f_2,...,f_K\}$. Set $\mathbf N=\{\mathbf{N_C}, \mathbf{N_G}\}$.% we can denote (\ref{Q'}) as:%\todo{why?}
%\begin{equation}
%\label{Q}
%G=Q(\mathbf N)
%\end{equation}
The process (\ref{X}) could be described as: %\todo{why we need this? }
\begin{equation}
\label{G2X}
p_{\theta_{N_X}}(X)=\int_{G}p_{\theta_{N_X}}(X|G)p(G)dG
\end{equation}
We can prove that causal disentanglement could lead to optimal solution, which can be formally described as:
\begin{theo}
\label{P1}
$\forall$ $K$ independent normal variables $N_1,...,N_K$, $\exists$ a function $Q$, $G=Q(\mathbf N)$, $\mathbf N=\{N_1,...,N_K\}$, which makes $p_{\theta_{N_X}}(X)$ equal to $p^{*}(X)$ under conditions of (\ref{p*}) and (\ref{G2X}).
\end{theo}





\begin{proof}
%\todo{rewrite the whole proof}
%The proof of Theorem\ref{T1} is in appendix.

%%%%%%%%
%%%%%%%%
%%%%%%%%

To prove Theorem\ref{P1}, we need two lemmas:
\begin{lemm}
\label{L1}
$\forall$ K dimension continuous variable $X=(X_1,...,X_K)$, if the support set of its joint probability density is a convex set in $R^K$, then $\exists$ K dimension independent uniform variables $U=(U_1,...,U_K)$ and a set of function $F=\{f_1,f_2,...,f_K\}$, which make $X=F(U)$ and $X_k=f_k(U_1,...,U_k)$, $k=1,2,...,K$.
\end{lemm}
The proof of Lemma\ref{L1} is provided by \citet{HePing}.

\begin{lemm}
\label{L2}
$\forall$ continuous variable $X$, set its distribution function as $f(X)=P(X \leq x)$, then $f(X) \sim U(0,1)$.
\end{lemm}
\begin{proof}
$P(f(X) \leq u)=P(X \leq f^{-1}(u))=f(f^{-1}(u))=u$
\end{proof}

%Based on these two lemmas, we can acquire such a theorem:
%\begin{theo}
%\label{T1}
%$\forall$ $K$ dimension continuous variable $Z=(Z_1,...,Z_K)$, $\exists$ $K$ dimentions independent normal variables $N=(N_1,...,N_K)$ and set of function $Q=\{q_1,...,q_K\}$, $Z=Q(N)$ and $Z_i=q_i(N_1,...,N_i)$, $i=1,2,...,K$. 
%\end{theo}
%\begin{proof}

Proof of Theorem\ref{P1} is equal to finding functions $q_i$, $i=1,2,...,K$, make $G_i=q_i(N_1,...,N_K)=C_i$.

Step 1: Because of Lemma\ref{L1}, we get that there exists independent uniform variables $(U_1,...,U_K)$ and function $F$ make $C=F(U)$, in which:
\begin{equation}
    U=(U_1,...,U_K)
\end{equation}
\begin{equation}
\label{fi}
    C_i=f_i(U_1,...,U_i)
\end{equation}

Set $U_i \sim U(a_i,b_i)$, $i=1,2,...,K$.

Step 2: Set there are arbitrary K independent normal variables $N_1,...,N_K$, $N_i \sim N(\mu_i,\sigma^2_i$). Set distribution function of $N_i$ is $g_i$, which means $g_i(x)=P(N_i \leq x)$. Denote:
\begin{equation}
\label{U'i}
    g_i(N_i)=U'_i, i=1,2,...,K
\end{equation}


Step 3: Because of Lemma\ref{L2}, $U'_1,...,U'_K$ are independent and they all are variables of uniform distribution $U(0,1)$.

Then $U_i$ in Step 1 can be represents by $U'_i$ as:
\begin{equation}
    U_i=(b_i-a_i)U'_i+a_i, i=1,2,...,K
\end{equation}
Because $g_i(N_i)=U'_i$ in (\ref{U'i}), which means $U'_i$ is function of $N_i$, so we can denote:
\begin{equation}
\label{hi}
    (b_i-a_i)U'_i+a_i=h_i(N_i)
\end{equation}


Step 4: Then we can find $C_i=q_i(N_1,...,N_K)$ as:
\begin{equation}
\label{qi}
    C_i=f_i(h_1(N_1),h_2(N_2),...,h_i(N_i))\\
    =q_i(N_1,...,N_K)\\
\end{equation}
In which set of $f_i$ is from equation \ref{fi} and $h_i$ is from equation \ref{hi}. Therefore, we can induce Theorem~\ref{P1} is right because $\forall$ $C$ (in equation (\ref{p*})), $\exists$ a function $Q$ makes $G=Q(\mathbf N)=\{q_i(N_1,...,N_K)\}_{i=1,2,...,K}$ (from equation (\ref{qi})) is equal to $C$ .
\end{proof}

Moreover, we have more general conclusion that:
\begin{remark}
\label{remark1}
$\forall$ $K$ dimension continuous variable $Z=(Z_1,...,Z_K)$, $\exists$ $K$ dimensions independent normal variables $N=(N_1,...,N_K)$ and set of function $Q=\{q_1,...,q_K\}$, $Z=Q(N)$ and $Z_i=q_i(N_1,...,N_i)$, $i=1,2,...,K$.
\end{remark}
The proof of Remark \ref{remark1} is in appendix.
%%%%%%%%
%%%%%%%%
%%%%%%%%
%With Theorem~\ref{T1}, we can induce Theorem~\ref{P1} because $\forall$ $C$ in (\ref{p*}), $\exists$ a function $Q$ (from Theorem~\ref{T1}) makes $G=Q(N)$ (in equation(\ref{G2X})) is equal to $C$.


%\end{proof}




\subsection{how to get this Q}\label{how to get Q}
%\todo{ set }\\
 We have proved that $\exists$ a function $Q$, $G=Q(\mathbf N)$, $\mathbf N=\{N_1,...,N_K\}$ in Theorem \ref{P1}. Now we propose how to find such $Q$:
\begin{theo}
\label{conditions}
 
%Condition 1: G is not independent\\
%condition 2: Q is not injective\\
Denote a set of $K$ functions of $K$ dimension vector as $\{Q'_i\}_{i=1,2,...,K}$, each $Q'_i: R^K \rightarrow R$, we can denote $G'_i = Q'_i(\mathbf b_i)=Q'_i(b_{i1},b_{i2},...,b_{iK})$. Denote $\{b_{ij}\}=B$, $B$ is $K \times K$ matrix. If $G'=\{Q'_i(\mathbf b_i)\}_{i=1,2,...,K}=G$ (in Theorem \ref{P1}), and $B$ can represented as $B=A \times \mathbf N'=A\times (N'_1,N'_2,...,N'_K)^T$ \todo{check}%(which can induce that $G'_i = Q'_i( (a_{i1},a_{i2},...,a_{iK})\times \mathbf N')$) 
under the conditions below:\\
Condition 1:  $A$ is $K \times K$ matrix which could be acquired through finite row exchanges of lower triangular matrix.\\
Condition 2: $\mathbf N'=(N'_1,N'_2,...,N'_K)^T$, $N'_1,N'_2,...,N'_K$ are independent normal variables.\\
Then we can get a solid solution of $\mathbf N'$:\\
$\mathbf N'=(N'_1,N'_2,...,N'_K)^T$, $\forall N'_i$, $\exists$ two real number $a_i$, $b_i$ and $N_k$ in $\mathbf N$(in Theorem \ref{P1}), makes $N'_i=a_i\times N_k+b_i$.\\
\end{theo}
The proof of Theorem \ref{conditions} is provided in appendix.
\todo{appendix}

Theorem \ref{conditions} tells us if $Q$ satisfies two conditions, we can ensure the solution of $\mathbf N$ is at least the linear transformer of true $\mathbf N$ when equaling $G=Q(\mathbf N)$.  


\subsection{The proposed linear solution}
%\todo{This is a draft, some assumption about causal layer would be check in the future}

\eat{
We are given an undirected, unweighted graph $\mathcal {G = (V, E)}$ with $ n = |\mathcal V|$ nodes with features. Denote the graph adjacency matrix as a $n \times n$ matrix $A$ and the node features as a $n \times d$ matrix $X$. Denote the degree matrix of $A$ as $D$.}

Now we consider to propose a method in an unweighted graph $\mathcal {G = (V, E)}$ with $ n = |\mathcal V|$ nodes with adjacency matrix $A_{n \times n}$ and the node features matrix $X_{n \times d}$.

Our method has 3 processes aiming to acquire $\mathbf N$, $G$ and $p_{\theta_{N_X}}(X)$ in Theorem \ref{P1} respectively, including encoder, causal layer and decoder.


\subsubsection{Encoder}
This process aims to acquire $\mathbf N$ in Theorem 4.1.  Because $N_1,N_2,...,N_K$ are independent, similar to Encoder of Variational Graph Auto-Encoder, we can acquire the distribution $q(\bm{\varepsilon}|(A,X))$ of latent variables $\bm{\varepsilon}$ (as equation (\ref{encoder})).% of which mean and covariance matrix are $\mu_{n \times K}=\{\mu_i\}_{i=1,2,...,n}$ and $\sigma_{n \times K\times K}=\{{diag(\sigma_i)_{K \times K}}\}_{i=1,2,...,n}$, $\sigma_i$ is $K$ dimensions vector.% Denote $\{\sigma_i\}_{i=1,2,...n}=\sigma'$, $\sigma'$ is a $n\times K$ matrix. %We can denote $\mu=\{\mu_i\}_{i=1,2,...,n}$, in which $\mu_i$ is $K$ dimensions vector., the covariance matrix is diagonal matrix, then $\sigma$ can be represented by $\sigma=\{{diag(\sigma_i)_{K \times K}}\}_{i=1,2,...,n}$, in which $\sigma_i$ is $K$ dimensions vector. We denote $\{\sigma_i\}_{i=1,2,...n}=\sigma'$, then $\sigma'$ is a $n\times K$ matrix, which could absolutely determine $\sigma$. 


  Moreover, $\varepsilon_i$ can satisfy the Condition 2 in Theorem \ref{conditions}, because the covariance matrix of each $\varepsilon_i$ is diagonal matrix, which makes them independent $K$ dimensions variables. Then $\mathbf N$(in Theorem 4.1) could be acquired by $\bm{\varepsilon}$ as $\mathbf N=(N_1,N_2,...,N_K)=\bm{\varepsilon}$.
 
\subsubsection{Causal layer}

This process aims to acquire $G$ in Theorem 4.1, in which we transforms independent variables $\bm{\varepsilon}$ into generative variables $G$ with causal structure.
Denote $\hat{G}$ as representation of the inverse matrix of generative factors $G$ in Theorem 4.1, as $\hat{G}_{K \times n}=G^T$. 

In this method, we consider linear SCM structure in $\hat{G}$, which means:
 \begin{equation}
\begin{aligned}
\label{G=CG+e}
\hat{G} = C^T\hat{G}+ \varepsilon^T %=(I-C^T)^{-1}\varepsilon^T
\end{aligned}
\end{equation}

Transform equation (\ref{G=CG+e}), then we have:
 \begin{equation}
\begin{aligned}
\hat{G} =(I-C^T)^{-1}\varepsilon^T
\end{aligned}
\end{equation}

Here $C_{K \times K}$ is an adjacency matrix of a directed acyclic graph (DAG) (because there is no circle in causal relationships), which is a parameters to be learnt in this layer. $\varepsilon^T$ represents noise variables in causal representation, and in this method it can be acquired by Encoder.  

Now we can prove that the$(I-C^T)^{-1}$ can satisfy Condition 1 in Theorem \ref{conditions}.

\todo{prove in appendix}

\subsubsection{Decoder}
This process aims to acquire $p_{\theta_{N_X}}(X)$ in Theorem \ref{P1}, which is to regenerate the adjacency matrix and features in graph $\mathcal {G = (V, E)}$. The process to regenerate the adjacency matrix is similar to Decoder of Variational Graph Auto-Encoder as equation (\ref{decoder}). Denote $G_i$ as the $i-th$ column in $\hat{G}$, $i=1,2,...,n$.

%\begin{equation}
%\begin{aligned}
%p(A \mid \hat{G})=\prod\prod   p\left(A_{j} \mid \hat{G}_{i}, %\hat{G}_{j}\right)
%\end{aligned}
%\end{equation}
 \begin{equation}
\begin{aligned}
p\left(A_{i j}=1| \hat{G}_{i}, \hat{G}_{j}\right)=\sigma\left(\hat{G}_{i}^{\top} \hat{G}_{j}\right)
\end{aligned}
\end{equation}
Regeneration of features is given by a nonlinear function, here we adopt an activate function:
 \begin{equation}
\begin{aligned}
p(X \mid \hat{G})= Elu(\hat{G})
\end{aligned}
\end{equation}

\subsubsection{Learning}

We adopt the ELBO band to shrink reconstruction loss between $p_{\theta_{N_X}}(X)$ and $p^{*}(X)$, and make $\varepsilon$ close to independent normal distribution:
\begin{equation}
\begin{aligned}
ELBO=E_{q(\hat{G}|A,X)}log(p(A|\hat{G}))\\+ KL(q(\bm{\varepsilon}|(A,X))|N(O,I))\\
\end{aligned}
\end{equation}
In addtion, we adopt $H(C)$ to let $C$ become a DAG:%\cite{b3} \cite{b4}, 
 \begin{equation}
\begin{aligned}
\label{DAG constrain}
H(C) = tr((I-\frac{c}{m}C\circ C)^n)-n
\end{aligned}
\end{equation}
$l_u$ is adopted for shrinking features reconstruction loss:
 \begin{equation}
\begin{aligned}
l_u = MSE(X,p(X|\hat{G}))
\end{aligned}
\end{equation}
Then the loss function is:
 \begin{equation}
\begin{aligned}
L=-E L B O+\alpha H(C)+\beta l_{u}\\
\end{aligned}
\end{equation}
In which $\alpha$ and $\beta$ are prior hyper-parameter.














% \begin{thebibliography}{00}
%     \bibitem{b1} F. Träuble et al., “On Disentangled Representations Learned from Correlated Data,” p. 12.
%     \bibitem{b2} R. Suter, Ð. Miladinovic, B. Schölkopf, and S. Bauer, “Robustly Disentangled Causal Mechanisms:  Validating Deep Representations for Interventional Robustness,” p. 10.
%     \bibitem{b3} He Ping. Independence Decomposition of Multidimensional Random Variables[J]. Proceedings of the 12th Annual Academic Conference of China Field Statistics Research Association, 2005

% \end{thebibliography}

